Semantically Interpretable and Controllable Filter Sets

In this paper, we generate and control semantically interpretable filters that are directly learned from natural images in an unsupervised fashion. Each semantic filter learns a visually interpretable local structure in conjunction with other filters. The significance of learning these interpretable filter sets is demonstrated on two contrasting applications. The first application is image recognition under progressive decolorization, in which recognition algorithms should be color-insensitive to achieve a robust performance. The second application is image quality assessment where objective methods should be sensitive to color degradations. In the proposed work, the sensitivity and lack thereof are controlled by weighing the semantic filters based on the local structures they represent. To validate the proposed approach, we utilize the CURE-TSR dataset for image recognition and the TID 2013 dataset for image quality assessment. We show that the proposed semantic filter set achieves state-of-the-art performances in both datasets while maintaining its robustness across progressive distortions.

==> Preprint for ArXiv/pcc.tex <==
\begin{table}[thb!]
\centering
\caption{Pearson correlation coefficients for different decolorization level}
\label{table:pcc}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\hline
\multirow{2}{*}{Metric} & \multicolumn{5}{c|}{Pearson Correlation Coefficient} \\ \cline{2-6} 
                        & Lv. 1      & Lv. 2      & Lv. 3     & Lv. 4     & Lv. 5     \\ \hline
PSNR-HMA                & 0.643      & 0.626      & 0.280     & 0.046     & 0.486     \\ \hline
MS-SSIM                 & 0.248      & 0.143      & 0.302     & 0.525     & 0.744     \\ \hline
SR-SIM                  & 0.370      & 0.260      & 0.301     & 0.497     & 0.732     \\ \hline
FSIMc                   & 0.391      & 0.253      & 0.303     & 0.553     & 0.778     \\ \hline
PerSIM                  & 0.126      & 0.085      & 0.304     & 0.554     & \textbf{0.804}     \\ \hline
AE(c+e)                 & 0.716      & 0.725      & 0.765     & 0.775     & 0.577     \\ \hline
AE(Weighted c+e)        & \textbf{0.772}      & \textbf{0.795}      & \textbf{0.801}     & \textbf{0.816}     & 0.730     \\ \hline
AE(L1)                  & 0.557      & 0.406      & 0.542     & 0.682     & 0.619     \\ \hline
AE(L2)                  & 0.079      & 0.004      & 0.275     & 0.454     & 0.568     \\ \hline\hline
\end{tabular}
\end{table}

==> Preprint for ArXiv/pcc_scc.tex <==
\begin{table}[thb!]
\centering
\caption{Pearson correlation coefficients and Spearman correlation coefficients for different decolorization level}
\label{table:pcc_scc}
%\begin{tabular}{|c|c|c|c|c|c|}
\begin{tabular}{|c| c c c c c|}
\hline
\hline
\multirow{2}{*}{Metric} & \multicolumn{5}{c|}{Pearson Correlation Coefficient} \\ \cline{2-6} 
                        & Lv. 1      & Lv. 2      & Lv. 3     & Lv. 4     & Lv. 5     \\ \hline
PSNR-HMA                & 0.643      & 0.626      & 0.280     & 0.046     & 0.486     \\ \hline
MS-SSIM                 & 0.248      & 0.143      & 0.302     & 0.525     & 0.744     \\ \hline
SR-SIM                  & 0.370      & 0.260      & 0.301     & 0.497     & 0.732     \\ \hline
FSIMc                   & 0.391      & 0.253      & 0.303     & 0.553     & 0.778     \\ \hline
PerSIM                  & 0.126      & 0.085      & 0.304     & 0.554     & \textbf{0.804}     \\ \hline
AE                 & 0.716      & 0.725      & 0.765     & 0.775     & 0.577     \\ \hline
AE(L1)                  & 0.557      & 0.406      & 0.542     & 0.682     & 0.619     \\ \hline
AE(L2)                  & 0.079      & 0.004      & 0.275     & 0.454     & 0.568     \\ \hline
Sem-AE        & \textbf{0.772}      & \textbf{0.795}      & \textbf{0.801}     & \textbf{0.816}     & 0.730     \\
\hline\hline
\multirow{2}{*}{Metric} & \multicolumn{5}{c|}{Spearman Correlation Coeffcieint}                        \\ \cline{2-6} 
                        & Lv. 1          & Lv. 2          & Lv. 3          & Lv. 4          & Lv. 5          \\ \hline
PSNR-HMA                & 0.505          & 0.475          & 0.140          & 0.229          & 0.732          \\ \hline
MS-SSIM                 & 0.471          & 0.345          & 0.111          & 0.224          & 0.691          \\ \hline
SR-SIM                  & 0.505          & 0.401          & 0.098          & 0.234          & 0.732          \\ \hline
FSIMc                   & 0.432          & 0.347          & 0.013          & 0.395          & 0.793          \\ \hline
PerSIM                  & 0.306          & 0.160          & 0.143          & 0.479          & \textbf{0.825} \\ \hline
AE                 & 0.648          & 0.764          & 0.795          & 0.786          & 0.389          \\ \hline

AE(L1)                  & 0.451          & 0.378          & 0.541          & 0.660          & 0.480          \\ \hline
AE(L2)                  & 0.084          & 0.120          & 0.188          & 0.381          & 0.543          \\ \hline
Sem-AE        & \textbf{0.725} & \textbf{0.815} & \textbf{0.802} & \textbf{0.797} & 0.615          \\ \hline\hline
\end{tabular}
\end{table}

==> Preprint for ArXiv/scc.tex <==

\begin{table}[thb!]
\centering
\caption{Spearman correlation coefficients for different decolorization level}
\label{table:scc}
\begin{tabular}{|c|c|c|c|c|c|}
\hline\hline
\multirow{2}{*}{Metric} & \multicolumn{5}{c|}{Spearman Correlation Coeffcieint}                        \\ \cline{2-6} 
                        & Lv. 1          & Lv. 2          & Lv. 3          & Lv. 4          & Lv. 5          \\ \hline
PSNR-HMA                & 0.505          & 0.475          & 0.140          & 0.229          & 0.732          \\ \hline
MS-SSIM                 & 0.471          & 0.345          & 0.111          & 0.224          & 0.691          \\ \hline
SR-SIM                  & 0.505          & 0.401          & 0.098          & 0.234          & 0.732          \\ \hline
FSIMc                   & 0.432          & 0.347          & 0.013          & 0.395          & 0.793          \\ \hline
PerSIM                  & 0.306          & 0.160          & 0.143          & 0.479          & \textbf{0.825} \\ \hline
AE(C+E)                 & 0.648          & 0.764          & 0.795          & 0.786          & 0.389          \\ \hline
AE(Weighted C+E)        & \textbf{0.725} & \textbf{0.815} & \textbf{0.802} & \textbf{0.797} & 0.615          \\ \hline
AE(L1)                  & 0.451          & 0.378          & 0.541          & 0.660          & 0.480          \\ \hline
AE(L2)                  & 0.084          & 0.120          & 0.188          & 0.381          & 0.543          \\ \hline\hline
\end{tabular}
\end{table}

==> pcc.tex <==
\begin{table}[thb!]
\centering
\caption{Pearson correlation coefficients for different decolorization level}
\label{table:pcc}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\hline
\multirow{2}{*}{Metric} & \multicolumn{5}{c|}{Pearson Correlation Coefficient} \\ \cline{2-6} 
                        & Lv. 1      & Lv. 2      & Lv. 3     & Lv. 4     & Lv. 5     \\ \hline
PSNR-HMA                & 0.643      & 0.626      & 0.280     & 0.046     & 0.486     \\ \hline
MS-SSIM                 & 0.248      & 0.143      & 0.302     & 0.525     & 0.744     \\ \hline
SR-SIM                  & 0.370      & 0.260      & 0.301     & 0.497     & 0.732     \\ \hline
FSIMc                   & 0.391      & 0.253      & 0.303     & 0.553     & 0.778     \\ \hline
PerSIM                  & 0.126      & 0.085      & 0.304     & 0.554     & \textbf{0.804}     \\ \hline
AE(c+e)                 & 0.716      & 0.725      & 0.765     & 0.775     & 0.577     \\ \hline
AE(Weighted c+e)        & \textbf{0.772}      & \textbf{0.795}      & \textbf{0.801}     & \textbf{0.816}     & 0.730     \\ \hline
AE(L1)                  & 0.557      & 0.406      & 0.542     & 0.682     & 0.619     \\ \hline
AE(L2)                  & 0.079      & 0.004      & 0.275     & 0.454     & 0.568     \\ \hline\hline
\end{tabular}
\end{table}

==> scc.tex <==

\begin{table}[thb!]
\centering
\caption{Spearman correlation coefficients for different decolorization level}
\label{table:scc}
\begin{tabular}{|c|c|c|c|c|c|}
\hline\hline
\multirow{2}{*}{Metric} & \multicolumn{5}{c|}{Spearman Correlation Coeffcieint}                        \\ \cline{2-6} 
                        & Lv. 1          & Lv. 2          & Lv. 3          & Lv. 4          & Lv. 5          \\ \hline
PSNR-HMA                & 0.505          & 0.475          & 0.140          & 0.229          & 0.732          \\ \hline
MS-SSIM                 & 0.471          & 0.345          & 0.111          & 0.224          & 0.691          \\ \hline
SR-SIM                  & 0.505          & 0.401          & 0.098          & 0.234          & 0.732          \\ \hline
FSIMc                   & 0.432          & 0.347          & 0.013          & 0.395          & 0.793          \\ \hline
PerSIM                  & 0.306          & 0.160          & 0.143          & 0.479          & \textbf{0.825} \\ \hline
AE(C+E)                 & 0.648          & 0.764          & 0.795          & 0.786          & 0.389          \\ \hline
AE(Weighted C+E)        & \textbf{0.725} & \textbf{0.815} & \textbf{0.802} & \textbf{0.797} & 0.615          \\ \hline
AE(L1)                  & 0.451          & 0.378          & 0.541          & 0.660          & 0.480          \\ \hline
AE(L2)                  & 0.084          & 0.120          & 0.188          & 0.381          & 0.543          \\ \hline\hline
\end{tabular}
\end{table}
